Hardness of approximation for strip packing

Strip packing is a classical packing problem, where the goal is to pack a set of rectangular objects into a strip of a given width, while minimizing the total height of the packing. The problem has multiple applications, e.g. in scheduling and stock-cutting, and has been studied extensively. When the dimensions of objects are allowed to be exponential in the total input size, it is known that the problem cannot be approximated within a factor better than $3/2$, unless $\mathrm{P}=\mathrm{NP}$. However, there was no corresponding lower bound for polynomially bounded input data. In fact, Nadiradze and Wiese [SODA 2016] have recently proposed a $(1.4 + \epsilon)$ approximation algorithm for this variant, thus showing that strip packing with polynomially bounded data can be approximated better than when exponentially large values in the input data are allowed. Their result has subsequently been improved to a $(4/3 + \epsilon)$ approximation by two independent research groups [FSTTCS 2016, arXiv:1610.04430]. This raises a question whether strip packing with polynomially bounded input data admits a quasi-polynomial time approximation scheme, as is the case for related two-dimensional packing problems like maximum independent set of rectangles or two-dimensional knapsack. In this paper we answer this question in negative by proving that it is NP-hard to approximate strip packing within a factor better than $12/11$, even when admitting only polynomially bounded input data. In particular, this shows that the strip packing problem admits no quasi-polynomial time approximation scheme, unless $\mathrm{NP} \subseteq \mathrm{DTIME}(2^{\mathrm{polylog}(n)})$.

==> approx.tex <==
\section{A $(4/3 + \epsilon)$-approximation Algorithm}

In this section we will present a $(4/3+\epsilon)$-approximation algorithm for the strip packing problem for polynomially bounded input data. The algorithm is a modification of the algorithm of Nadiradze and Wiese \cite{NW16}, which obtained a $(1.4+\epsilon)$-approximation.

The high-level idea of the algorithm is as follows. We partition the input items in several classes, which will then be considered separately. This includes large items (i.e., items which are large in both dimensions), vertical and horizontal (i.e., large in exactly one dimension), and small items (i.e., small in both dimensions). We show that we can round the heights of the large and vertical items to only $O_\epsilon(1)$ different sizes. We then show that there exists a partition of a rectangular area of size $W \times (4/3+\epsilon) OPT$ into $O_\epsilon(1)$ rectangular boxes, where each box can also be large, horizontal, or vertical, and such that we can pack all large items into the large boxes, all vertical items into the vertical boxes of exactly the same height, and all horizontal items into the horizontal boxes.

The algorithm starts by guessing the value of $OPT$, and guessing the partition which satisfies the required properties. It then inserts the large items into the corresponding large areas, puts the vertical items greedily into the areas of the corresponding height, and then puts the horizontal items into the horizontal boxes using linear programming. At the end, it inserts the small items into the empty areas.

This follows the approach of Nadiradze and Wiese \cite{NW16}. However, by a more careful analysis of how the vertical items can be rearranged, we obtain a better approximation ratio.

For simplicity of the description, we will show a $(4/3+O(\epsilon))$-approximation algorithm. It can be modified to a $(4/3+\epsilon)$-approximation algorithm by scaling down the parameter $\epsilon$ by an appropriate constant.

%------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Partitioning Input Items into Classes}\label{subsec:item-classes}

In the algorithm we will use parameters $\delta > \mu$ which will depend on $\epsilon$, and the value of which will be fixed later. 

\begin{lemma}\label{lem:estimating-opt}
By losing an $(1+\epsilon)$ factor in the value of the objective, we can assume that we know the value of $OPT$.
\end{lemma}

Similarly as in \cite{NW16}, we partition the input items $I$ into the following groups:
%To get a better approximation ratio, we had to change the lower bound for the tall items.
\begin{itemize}
\item large items $L$; $i \in L$ if $w_i \ge \delta W$ and $h_i \ge \delta OPT$,
\item tall items $T$; $i \in T$ if $w_i < \delta W$ and $h_i > OPT / 3$,
\item vertical items $V$; $i \in V$ if $w_i < \mu W$ and $OPT/3 \ge h_i \ge \delta OPT$,
\item horizontal items $H$; $i \in H$ if $w_i \ge \delta W$ and $h_i < \mu OPT$,
\item small items $S$; $i \in S$ if $w_i < \mu W$ and $h_i < \mu OPT$,
\item medium items $M$; $M = I \setminus (L \cup T \cup V \cup H \cup S)$.
\end{itemize}

We can show that we can round the values of the $y$-coordinates of all the items within $L \cup T \cup V$.

\begin{lemma}\label{lem:rounding-verticals}
By losing an $(1+\epsilon)$ factor in the value of the objective, we can assume that each item in $L \cup T \cup V$ has height which is a multiplicity of $\epsilon \delta OPT$. We can consider only solutions in which the $y$-coordinates of all items in $L \cup T \cup V$ are multiples of $\epsilon \delta OPT$.
\end{lemma}

From now on we will assume that all items in $L \cup T \cup V$ satisfy conditions of Lemma \ref{lem:rounding-verticals}. As in \cite{NW16}, we can show that when choosing the parameters $\delta$ and $\mu$ appropriately, the medium elements $M$ can be packed into two small boxes.

\begin{lemma}\label{lem:delta-mu}
There is a choice of parameters $\delta$ and $\mu$, which can be computed in polynomial time, and which satisfies:
\begin{itemize}
\item $1 \ge \delta > \mu \ge \Omega_\epsilon(1)$,
\item $\mu \le (\delta \epsilon)^{O_\epsilon(1)}$,
\item all items in $M$ can be packed in polynomial time into boxes of size $W \times \epsilon OPT$ and $\epsilon W/3 \times OPT/3$.
\end{itemize}
\end{lemma}

The algorithm chooses the parameters $\delta$ and $\mu$ so that conditions of Lemma \ref{lem:delta-mu} are satisfied.

%------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Partitioning into Boxes -- First Level} 
We now present the first partition of the area $W \times OPT$ into rectangular boxes, which has some nice properties. This partition will then be refined in the next subsection. Our partition is similar to the partition from  Lemma 3.2 of \cite{NW16}, but we obtain it in a much simpler way. In particular, we do not use the corridor decomposition machinery from \cite{AW13}.

\begin{theorem}\label{thm:partition-1}
Consider an optimal solution for an instance of the strip packing problem. There exists a decomposition of the area $W \times OPT$ into rectangular boxes with integer coordinates satisfying the following conditions:
\begin{itemize}
\item the number of boxes is at most $K = 5/(\epsilon \delta)^2$,
\item for each item in $L$ there is a box containing exactly this item,
\item each box which does not contain an element of $L$ has either a height of $\epsilon \delta OPT$ (horizontal), or a width of at most $\epsilon \delta W$ (vertical box),
\item each item in $T \cup V$ is contained in the union of vertical boxes, and each item in $H$ is contained in the union of horizontal boxes,
\item each item in $T \cup V \cup H$ can be intersected by a boundary of a box only along its longer edge.
\end{itemize}
\end{theorem}

\begin{proof}
Due to Lemma \ref{lem:rounding-verticals} we can assume that in the solution all items from $L \cup T \cup V$ have height which is a multiplicity of $\epsilon \delta OPT$, and have y-coordinates which are also multiples of $\epsilon \delta OPT$. We partition the box $W \times OPT$ into \emph{cells} of size $\epsilon \delta OPT \times \epsilon \delta W$. Then the top and the bottom edge of the items from $L \cup T \cup V$ all lie on horizontal lines between the cells (see Figure \ref{fig:partition-level1}a). 

We now create the partition as follows. For each large item $i_L \in L$ we add to the partition a \emph{large box} containing exactly the item $i_L$ (i.e., the boundary of the box is formed by the edges of $i_L$). Now, we consider one by one all cells $C$ which are not covered by large items. Notice that any such cell can be intersected by at most two large items: one containing the left boundary edge of the cell, and one containing the right boundary edge of the cell. If $C$ has non-empty intersection with the large items, we only consider the part of $C$ which is not covered by the large items, instead of the full cell $C$. We consider all items from $T \cup V \cup H$ intersecting $C$. If $C$ is not intersected by any item from $T \cup V$, we say that $C$ is a \emph{horizontal cell}, and the top and the bottom edges of $C$ will be boundaries of a horizontal box, i.e., we add these edges as the edges of the partition. If $C$ is intersected by items from $T \cup V$, but not by items of $H$, we say that $C$ is a \emph{vertical cell}, and the left and right edges of $C$ will be boundaries of a vertical box. In the remaining case, $C$ is intersected both by items of $T \cup V$ and $H$. Then, as all items of $T \cup V$ cross the whole cell, we find the leftmost and the rightmost edge of the cell separating the vertical and horizontal items in the cell, and we add them to the partition, separating the cell into a \emph{vertical fragment} and at most two \emph{horizontal fragments}. For the horizontal fragments, we additionally add the corresponding fragments of the top and bottom boundaries of the cells to the partition. We get a partition as pictured in Figure \ref{fig:partition-level1}b. 

\begin{figure}[t]
  \centering
  \includegraphics[width=\textwidth]{figures/partition-level1}
  \caption{\label{fig:partition-level1}The first level of the partition. The grey rectangles represent the input items. a) Decomposition of the area $W \times OPT$ into cells. b) First step of the partition. Here we obtain large boxes and horizontal boxes, but the shape of the vertical pieces can be more complicated. c) Refining the partition to obtain vertical boxes.
  }
\end{figure}

Each piece of the partition either corresponds to a large item of $I$, or it is a union of horizontal cells and horizontal fragments (in which case it is a rectangle of height $\epsilon \delta OPT$, called a \emph{horizontal box}), or it is a union of vertical cells and vertical fragments. In the last case the piece of the partition is contained inside a vertical strip of width $\epsilon \delta W$, but it can be a rectilinear polygon with $O(1/(\epsilon \delta))$ edges, instead of a rectangle. To further partition each such polygon into a collection of rectangles, we extend each vertical edge of the polygon within the interior of the polygon, until it hits the boundary of the polygon. That partitions the pieces into rectangles called \emph{vertical boxes}, and we get a partition of the area $W \times OPT$ into rectangular boxes, as pictured in Figure \ref{fig:partition-level1}c. 

We now have to show that the partition satisfies all requirements of the lemma statement. We first bound the number of boxes of the partition. From the definition of a large item, the number of large boxes is at most $1/\delta^2$. As the number of cells is $1/(\epsilon \delta)^2$, both the number of the vertical boxes and the horizontal boxes can be up to $2/(\epsilon \delta)^2$. The total number of boxes is therefore at most $K = 5/(\epsilon \delta)^2$.

Clearly, for each item in $L$ there is a box containing exactly this item. Any box which does not contain an item of $L$ is either a horizontal box or a vertical box, and therefore it has height of $\epsilon \delta OPT$ or width of at most $\epsilon \delta W$. Each horizontal (vertical) cell or horizontal (vertical) fragment can contain only items of $H$ ($V \cup T$), therefore each item in $T \cup V$ is contained in the union of vertical boxes, and each item in $H$ is contained in the union of horizontal boxes. As the horizontal edges of the partition can intersect only items of $H$, and vertical edges of the partition can intersect only items of $V \cup T$, each item in $T \cup V \cup H$ can be intersected by a boundary of a box only along its longer edge.
\end{proof}

%------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Partitioning into Boxes -- Second Level} 

Here we show the construction of the final partition of an area $W \times (4/3 + O(\epsilon)) OPT$ into a small number of rectangular boxes, for which there is a packing of the items such that no item is crossed by the boundaries of the boxes, and the items of various types are nicely grouped. This partition will then be used by the algorithm. Our partition has similar properties to the one obtained in Theorem 2.1 of \cite{NW16}, however, we are able to make it within a smaller area, which results in a better approximation ratio of the algorithm. Also, in our construction the number of boxes of the partition is polynomial in $1/\epsilon$ and $1/\delta$, instead of being exponential as in \cite{NW16}.

\begin{theorem}\label{thm:partition-2}
Consider an instance of the strip packing problem, for which there exists a solution with the objective value $OPT$. There exists a partition of the area $W \times (4/3 + O(\epsilon)) OPT$ into rectangular boxes with integer coordinates, and a corresponding solution with the objective value $(4/3 + O(\epsilon)) OPT$, satisfying the following conditions:
\begin{itemize}
\item the number of boxes is at most $K' = O(1/(\epsilon^6 \delta^7))$,
\item for each item in $L$ there is a box containing only this item,
\item there are two boxes of sizes $W \times \epsilon OPT$ and $\epsilon W/3 \times OPT/3$ containing all items in $M$, and no other items,
\item each item $i \in T \cup V$ of some height $h_i$ is contained in a vertical box of height exactly $h_i$,
\item each item in $H$ is contained in a horizontal box.
\end{itemize}
\end{theorem}

We start with the partition obtained from Theorem \ref{thm:partition-1}. From Lemma \ref{lem:delta-mu} we know that we can pack the items of $M$ into the required boxes of small size. These boxes will then be placed on top of the current partition. To show the existence of a partition with the above properties, we have to deal with two issues. The first one are items of $V \cup T \cup H$ overlapping the boundaries of the partition from Theorem \ref{thm:partition-1}. The items of $V \cup H$ are easy to handle, as we show in Lemma \ref{lem:moving-h-and-v} (which is similar to Lemmas 3.3 and 3.5 in \cite{NW16}). The items of $T$ are more difficult to deal with, and they will require modifying the partition into boxes. Also, we will have to create a partition within the vertical boxes, so that the items of $T \cup V$ become grouped as required by the lemma statement. While constructing the new partition, some items will be placed into newly constructed boxes, which will be placed on top of the current partition. So far, that follows the ideas from \cite{NW16}.

\begin{lemma}\label{lem:moving-h-and-v}
Consider an instance of the strip packing problem, and a partition for it as given by Theorem \ref{thm:partition-1}. Let $V' \subseteq V$ and $H' \subseteq H$ be the sets of vertical and horizontal items intersected by the lines of the partition. Then all items from $H'$ can be packed into a box of size $W \times \epsilon OPT$. All items of $V'$ can be packed into at most $1/(\epsilon \delta)$ boxes s.t. each $i \in V'$ is inside a box of height $h_i \le OPT/3$, and the total width of the boxes is at most $\epsilon W/3$.
\end{lemma}

We now have to deal with a collection of tall items $T' \subseteq T$ which overlap the boundary of the partition. These items have small total area, but we cannot remove them to the top of our partition, as their height is too large. Instead, each such item will be treated in the same way as the large items, i.e., it will have its own box of the partition. We can do that, as the number of items of $T$ is upper bounded by $2K / \delta = 10/(\epsilon^2 \delta^3)$. That follows the ideas from \cite{NW16}.

We will now show a way of rearranging the items of $V \cup T$ within the vertical boxes, and also using some newly-created boxes, so that the items are grouped w.r.t. their heights, and the items of $T'$ are not moved. That will allow us to create a box partition as required by Theorem \ref{thm:partition-2}. We do that in the following steps. First, we will show how to perform this rearrangement if we have only items of $T$. In the next step, we will allow items of $V$, but we will assume that all of them have unit width. In the last step, we will show how to extend the reasoning to work for arbitrary items $V$. That still follows the same high-level idea as in \cite{NW16}, but we will make the partition in a slightly different way. In particular, we will remove a smaller number of items to the newly-created boxes, which will allow us to fit the extra boxes inside an area of $(1-\epsilon) W \times OPT/3$, which will then lead to a $(4/3 + \epsilon)$-approximation  algorithm. Also, in our construction, the number of boxes of the partition is polynomial in $\epsilon$ and $\delta$.

\paragraph{Dealing with tall items only.}

For now let us consider only the tall items intersecting some vertical box $B$. We can show the following result. In the following proof, the idea of partitioning the items of $T$ into top items $T^t$ and bottom items $T^b$, and trying to group the items within both $T^t$ and $T^b$ into a small number of boxes, is taken from \cite{NW16}. However, we group the items in a different way, obtaining the number of boxes which is polynomial in $\epsilon$ and $\delta$.

\begin{lemma}\label{lem:rearranging-top}
Let $B$ be a vertical box, and $T_B$ a collection of tall items which have non-empty intersection with $B$. Then the items of $T_B$ can be rearranged within $B$ in such a way that (i) they can be partitioned into at most $14/(\epsilon^2 \delta^2)$ boxes, where each box is of some height $h$ and contains only items of height $h$, and (ii) the items of $T_B$ which are not completely contained in $B$ are not moved.
\end{lemma}

\begin{proof}
Denote by $T'$ the items of $T_B$ which are not completely contained in $B$. We have $|T'| \le 4$, as at most two tall items can intersect each vertical edge of $B$. Each vertical line can intersect at most two items of $T_B$, and we can partition $T_B$ into \emph{top items} $T^t$ and \emph{bottom items} $T^b$ (see Figure \ref{fig:rearranging-top}a). We now shift all items of $T^t \setminus T'$ upwards, until the top boundary of the item touches the top boundary of $B$. Similarly, we shift all items of $T^b \setminus T'$ downwards, until the bottom boundary of the item touches the bottom boundary of $B$ (see Figure \ref{fig:rearranging-top}b). Next, we would like to shift the items within $T^t \setminus T'$ and $T^b \setminus T'$ horizontally, so that the items of the same height would be grouped together, and so that the top items do not overlap with the bottom items. If $T' = \emptyset$, we can get a solution with at most $2/(\epsilon \delta)$ boxes as follows. We sort the top items non-increasingly and the bottom items non-decreasingly, as can be seen in Figure Figure \ref{fig:rearranging-top}c. It is then easy to show that the top items and the bottom items do not overlap, as they didn't overlap before the sorting operation. However, due to items in $T'$, which cannot be shifted, we have to arrange the items of $T^t$ and $T^b$ in a more complex manner.

\begin{figure}[t]
  \centering
  \includegraphics[width=.8\textwidth]{figures/rearranging-top}
  \caption{\label{fig:rearranging-top} Rearranging the items of $T$ within a vertical box, when $T' = \emptyset$. a) Partitioning the tall items into $T^t$ (dark grey) and $T^b$ (light grey). b) Shifting the items towards the top and bottom edge of the box. c) Sorting the shifted items.
  }
\end{figure}

By increasing the number of vertical boxes at most by a factor of $3$, we can assume that there are at most two items in $T'$, and that $T' \subseteq T^b$. For that, we cut each box $B$ along the (at most two) vertical lines corresponding to the edges of the items of $T' \cap T^t$ which are inside $B$. That partitions the box into at most three smaller boxes. In the "middle" box we clearly have $T' \cap T^t = \emptyset$. In the "outside" boxes, after cutting out separate faces for the items in $T'$, all items are bottom items.
 
We proceed with the rearrangement as follows.  Let $b_\ell \in T'$ be the item overlapping the left boundary of $B$, and let $d_\ell$ be the distance from the top edge of $b_\ell$ to the bottom edge of $B$. Assume w.l.o.g. that $d_\ell \ge d_r$ (as otherwise we would consider the item intersecting the right boundary of $B$ instead of $b_\ell$). Consider a horizontal line $h$ coincident with the top boundary of $b_\ell$. Let $t_t \in T^t$ be the leftmost item of $T^t$ which intersects the line $h$. We consider the following cases.

\begin{figure}[t]
  \centering
  \includegraphics[width=\textwidth]{figures/partition-1}
  \caption{\label{fig:partition-1}Partitioning a vertical box into smaller boxes. In a) the horizontal line $h$ intersects some items of $T^t$, and the leftmost of these items is $t^t$. In b), the horizontal line $h$ does not intersect any items of $T^t$.}
\end{figure}


Assume first that such item $t_t$ exists (see Figure \ref{fig:partition-1}a). Let $v^t_\ell$ and $v^t_r$ be the vertical lines coincident with the left and right edges of $t_t$, respectively. Let $b_1, b_2 \in T^b$ be the items intersected by the corresponding lines  $v^t_\ell$ and $v^t_r$. Note that possibly no items $b_1, b_2$ exist. We will now partition the box $B$ into two boxes, $B_\ell$ and $B_r$, along the vertical line $v^t_r$, where the box $B_\ell$ is to the left of $B_r$. We will rearrange the items within $B_\ell$ so that they can be put into at most $7/(\epsilon \delta)$ boxes satisfying the conditions of the lemma statement. We will then recursively continue with the box $B_r$, where now the item $b_2$ intersects the left edge of the box. Notice that the value of $d_\ell$ for the box decreased: $d_\ell$ is the distance from the line $h$ to the bottom edge of $B$. As $t_t$ intersects $h$, and $b_2$ does not intersect $t_t$, the distance from the top edge of $b_2$ to the bottom edge of $B$ must be smaller than $d_\ell$. That gives us that we can continue the following operation for at most $2/(\epsilon \delta)$ steps, as then we cannot decrease the value of $d_\ell$ or $d_r$ any further.

Now let us define how we make the rearrangement within the box $B_\ell$. Let $b_0 \in T^b$ be the highest item in $T_b$, contained between $b_\ell$ and $b_1$. Possibly $b_0 = b_\ell$. We proceed as follows. Let $v^b_\ell$ and $v^b_r$ be the vertical lines coincident with the left and right edges of $b_0$, respectively. Let $t_1, t_2 \in T^t$ be the items intersected by the corresponding lines  $v^b_\ell$ and $v^b_r$. Possibly no items $t_1, t_2$ exist. We will now partition the items of $T^b$ and $T^t$ intersecting the box $B_\ell$ as follows. $T^b = T^b_0 \cup T^b_1 \cup T^b_2 \cup \{b_\ell, b_0, b_1,b_2\}$, where $T^b_0$ are the items contained between $b_\ell$ and $b_0$, $T^b_1$ are the ones between $b_0$ and $b_1$, and $T^b_2$ are the ones between $b_1$ and $b_2$. $T^t = T^t_0 \cup T^t_1 \cup T^t_2 \cup \{t_1,t_2, t_t\}$, where $T^t_0$ are the items to the left of $t_1$, $T^t_1$ are between $t_1$ and $t_2$, and $T^t_2$ are between $t_2$ and $t_t$. We now sort the items of $T^t_0$, $T^t_1$, $T^b_1$ and $T^b_2$ non-increasingly, and the items of $T^t_2$ and $T^b_0$ non-decreasingly. That yields a partition into at most $7/(\epsilon \delta)$ boxes.

We now have to show that after sorting the top and the bottom items do not intersect. The only non-trivial parts are showing that the items of $\{b_\ell\} \cup T^b_0$ do not intersect with $T^t_0 \cup \{t_1\}$, and that $T^b_1 \cup \{b_1\}$ do not intersect with $\{t_2\} \cup T^t_2$. First, notice that the items $b_1, b_\ell$ are not intersected by any items of $T^t_0 \cup T^t_2$, as none of these items intersects the horizontal line $h$. Next, notice that the items $t_1, t_2$ are not intersected by any items of $T^b_0 \cup T^b_1$, as none of these items is higher than $b_0$, and $b_0$ does not intersect $t_1, t_2$. As to the remaining elements, we argue as follows. Assume for now, that we decide to cut the items $b_\ell, b_1, t_1, t_2$ along the corresponding lines: the left boundary of $B$, $v^t_\ell, v^b_\ell, v^b_r$. Then, instead of keeping these items in their original position, we sort the cut part of the corresponding item together with all other items. Then, as in the case when $T' = \emptyset$, after sorting the top and the bottom items do not overlap. Now, as the cut items do not get sorted but they stay at the place of the smallest items, the height profile of the other items can only decrease, which does not create any intersections.
 
We now consider the case that no item  $t_t$ exists (see Figure \ref{fig:partition-1}b), i.e., no item of $T^t$ intersects the horizontal line $h$. Let $b_r \in T^b$ be the item which intersects the right boundary of $B$. Possibly $b_r$ does not exist, but if it exists then we know that it doesn't intersect the line $h$. We proceed similarly as before. Let $b_0$ be the highest item in $T^b$, where possibly $b_0 = b_\ell$. Let Let $v^b_\ell$ and $v^b_r$ be the vertical lines coincident with the left and right edges of $b_0$, respectively. Let $t_1, t_2 \in T^t$ be the items intersected by the corresponding lines  $v^b_\ell$ and $v^b_r$. Possibly no items $t_1, t_2$ exist. We will partition the items of $T^b$ and $T^t$ intersecting the box $B$ as follows. $T^b = T^b_0 \cup T^b_1 \cup \{b_\ell, b_0,b_r\}$, where $T^b_0$ are the items contained between $b_\ell$ and $b_0$, and $T^b_1$ between $b_0$ and $b_r$. $T^t = T^t_0 \cup T^t_1 \cup T^t_2 \cup \{t_1,t_2\}$, where $T^t_0$ are the items to the left of $t_1$, $T^t_1$ are between $t_1$ and $t_2$, and $T^t_2$ are to the right of $t_2$. We now sort the items of $T^t_0$, $T^t_1$ and $T^b_1$ non-increasingly, and the items of $T^t_2$ and $T^b_0$ non-decreasingly. That yields a partition of $B$ into at most $6/(\epsilon \delta)$ boxes.

Again, we have to show that after sorting the top and the bottom items do not intersect, i.e., that the items of $\{b_\ell\} \cup T^b_0$ do not intersect with $T^t_0 \cup \{t_1\}$, and that $T^b_1 \cup \{b_r\}$ do not intersect with $\{t_2\} \cup T^t_2$. First, notice that the items $b_\ell, b_r$ are not intersected by any items of $T^t_0 \cup T^t_2$, as none of these items intersects the horizontal line $h$. Next, notice that the items $t_1, t_2$ are not intersected by any items of $T^b_0 \cup T^b_1$, as none of these items is higher than $b_0$, and $b_0$ does not intersect $t_1, t_2$. As to the remaining elements, we argue as before. Assume for now, that we decide to cut the items $b_\ell, b_r, t_1, t_2$ along the corresponding lines: the left boundary of $B$, the right boundary of $B$, $v^b_\ell, v^b_r$. Then, instead of keeping these items in their original position, we sort the cut part of the corresponding item together with all other items. Then, as in the case when $T' = \emptyset$, after sorting the top and the bottom items do not overlap. Now, as the cut items do not get sorted but they stay at the place of the smallest items, the height profile of the other items can only decrease, which does not create any intersections.

The total number of boxes created in this way within the original box $B$ is at most $14/(\epsilon^2 \delta^2)$. 
\end{proof}

\paragraph{Adding unit width vertical items.}
Now, we allow vertical items $V$ within a vertical box $B$, but we assume that each of the vertical items has unit width (while all the items have integral coordinates). We will present a decomposition into boxes in this setting, such that the boxes satisfy the statement of Theorem \ref{thm:partition-2}. There will be two main changes compared to the result from Lemma \ref{lem:rearranging-top}. The first one is, that we will expand the height of the vertical box $B$ from $h(B)$ to $(1+O(\epsilon)) \cdot h(B)$, increasing the value of the objective by a $(1+O(\epsilon))$ factor. The second change is, that we will introduce an additional box of size $(1-\epsilon) w(B) \times h(B) /3$, and remove some items of $V$ from $B$ into the new box.

The following lemma allows us to obtain a better approximation factor than in \cite{NW16}. They show a similar result, but requiring an additional box of height $0.4 h(B)$ instead of $b(B)/3$. By increasing the height of the original box by a factor of $(1+O(\epsilon))$, we are able to remove a smaller number of items from $B$ to the additional box, and we can keep the height of the additional box smaller. It also allows us to fix a lower bound on the height of tall items on $OPT/3$ instead of $0.4 OPT$. That results in a better overall approximation factor.

\begin{lemma}\label{lem:rearranging-unit}
Let $B$ be a vertical box, and $T_B, V_B$ collections of tall and vertical items which have non-empty intersection with $B$, and such that all items in $V_B$ have unit width. Then all items of $T_B \cup V_B$ can be packed into two boxes, $B' \cup B''$, where $B'$ is a box of size $w(B) \times (1+2 \epsilon) h(B)$, and $B''$ is a box of size $(1-\epsilon) w(B) \times h(B) /3$, in such a way that (i) the items are grouped into at most $15/(\epsilon^4 \delta^5)$ boxes, where each box is of some height $h$ and contains only items of height $h$, and (ii) the items of $T_B$ which are not completely contained in $B$ are placed in $B'$, at the same coordinates as they were in $B$.
\end{lemma}

\begin{proof}
First, consider a rectangular box which has items from $V_B$ only. We will show that we can always rearrange the items in such a way, that they can be packed into at most $1/(\epsilon^2 \delta^3)$ boxes: First, within each vertical unit-width strip we sort the items from the highest to the smallest, and then place them on top of each other, starting from the bottom of the box. Then, we sort the strips in the following way. First, we maximize the number of the largest items, then of the second-largest items etc. As there are at most $1/(\epsilon \delta)$ different sizes of items in $V_B$, and there can be at most $1/\delta$ items on top of each other, all the items can then be packed into at most $1/(\epsilon^2 \delta^3)$ boxes.

We now proceed as follows. As before, we partition the tall items $T_B$ into the top items $T^t$ and the bottom items $T^b$, and we partition $B$ into at most $3$ boxes s.t. $|T'| \le 2$and $T' \subseteq T^b$. That doesn't intersect any items from $T_B$, as they all have unit width. We shift the tall items from $T^t$ ($T^b$) upwards (downwards) as before, this time exchanging them with the vertical items which were above (below) them.

Now, the vertical items which are not contained between two tall items can be all shifted upwards or downwards and "glued" into a single unit-width "pseudo-item" which will then be inserted into $T^t$ or $T^b$. Let $V'$ be the set of all vertical items that haven't been put into pseudo-items. For now we remove $V'$ from $B$. With the remaining items, we do the same operation as before, treating pseudo-items in the same way as tall items. That will now give us a partition into at most $14/(\epsilon^2 \delta^2)$ boxes. Now, each box can contain not only tall items, but also pseudo-items. We can group all of them together within one rectangular area, and partition them into at most $1/(\epsilon^2 \delta^3)$ boxes, as described above. We do the same with items which are contained in the area below items from $T'$. That gives us a partition of the items of $T_B \cup V_B \setminus V'$ into at most $14/(\epsilon^4 \delta^5)$ boxes.

We now have to add the items of $V'$ into the partition. Notice that, due to the choice of $V'$, these items are contained inside a rectangle $w(B) \times h(B) /3$. We want to place them inside the new box $B''$, and into the remaining spaces within $B'$. As before, we merge these items into unit-width "pseudo-items". We then consider a subset $V''$ of $\epsilon \cdot w(B)$ shortest pseudo-items. These will then be added into $B'$. The remaining items $V' \setminus V''$ fit inside the box $B''$ of size $(1-\epsilon) w(B) \times h(B) /3$, and can be rearranged within $B''$ into $1/(\epsilon^2 \delta^3)$ boxes.

The last step is showing how to fit the items $V''$ within $B'$. The items of $V''$ are grouped into pseudo-items, and let $h_0$ be the height of the highest pseudo-item. Let $a$ denote the total area of $B'$ which is not occupied by the items of $T_B \cup V_B \setminus V'$, and which is contained between the top and the bottom items. Due to the arrangement of the items, this area is partitioned into at most $14/(\epsilon^2 \delta^2)$ rectangular pieces. Due to the choice of $V''$, and expanding the height of the box by a factor of $(1+2\epsilon)$, we have $a \ge (1+\epsilon) w(B) \cdot h_0$. The items of $V''$ fit into a rectangle of size $\epsilon w(B) \times h_0$, and they can be rearranged within this rectangle into at most $1/(\epsilon^2 \delta^3)$ boxes. Therefore, we can find at most $14/(\epsilon^2 \delta^2) + 1/(\epsilon \delta) \le 15/(\epsilon^2 \delta^2)$ rectangular boxes, each of height $h_0$, with total width of $\epsilon w(B)$, which can be used for packing the items of $V''$. The number of boxes for the items of $V''$ will then increase to at most $1/(\epsilon^2 \delta^3) + 15/(\epsilon^2 \delta^2) \le 2/(\epsilon^2 \delta^3)$.
The total number of boxes within $B' \cup B''$ will be at most $15/(\epsilon^4 \delta^5)$.
\end{proof}

\paragraph{General case.}
Now, we allow arbitrary vertical items $V$. First, we slice the vertical items into unit-width items, and compute a partition into boxes by using Lemma \ref{lem:rearranging-unit}. Then, the original vertical items will be inserted greedily into the boxes created for the sliced items, plus a small number of additional boxes. We explain the details in the following proof. This part is similar as the corresponding part in \cite{NW16}.

\begin{proof}[Proof of Theorem \ref{thm:partition-2}]
Consider an optimal solution OPT for an instance of the strip packing problem. Consider a decomposition of the area $W \cdot OPT$ into at most $K$ rectangular boxes, as given by Theorem \ref{thm:partition-1}, and let $H',V'$ be the horizontal and the vertical items intersected by the lines of the partition. We remove them from the packing, and by Lemma \ref{lem:moving-h-and-v} we can place them into $1/(\epsilon \delta)$ boxes which together occupy an area of $W \cdot \epsilon OPT$ and $\epsilon W/3 \times OPT/3$. Also, by Lemma \ref{lem:delta-mu}, the medium items fit into boxes of size $W \times \epsilon OPT$ and $\epsilon W/3 \times OPT/3$.

We slice all vertical items $V$ into unit-width items, and for each vertical box of the decomposition make a finer partition into boxes, as given by Lemma \ref{lem:rearranging-unit}. All boxes of our final partition fit into an area of $W \times (4/3 + O(\epsilon) OPT)$ as follows. The original boxes, possibly expanded by a $(1+O(epsilon))$ factor in height, fit into a box of size $W \times (1+ O(\epsilon) OPT)$. On top of it, we place the boxes of size $W \times \epsilon OPT$ containing some of the medium items, and the items of $H'$. On top of it, within an area of $(1-\epsilon) W \times OPT/3$, we place all the additional boxes corresponding to the vertical boxes of the first decomposition. Next to it, we place two boxes of size $\epsilon/3 W \times OPT/3$ containing the remaining medium items, and the boxes for the items $V'$. We also have an empty box of size $(1-\epsilon) W \times OPT/3$, which we will use later.

Our partition consists of at most $3K \cdot 15/(\epsilon^4 \delta^5) \le 225/(\epsilon^6 \delta^7)$ boxes, and satisfies the conditions of Theorem \ref{thm:partition-2}, assuming that we allow the vertical items to be sliced. We now modify the packing, by taking out the sliced vertical items, putting them back into non-sliced items, and packing them greedily into the vertical boxes of the corresponding size. That leaves at most $225/(\epsilon^6 \delta^7)$ items of $V$ unassigned. They will now be assigned into new $1/(\epsilon \delta)$ boxes, and placed into a the spare area o size $\epsilon/3 W \times OPT/3$. We can do that, as their total width is at most $225/(\epsilon^6 \delta^7) \mu W \le \epsilon W /3$. The additional number of boxes will be $O(1/(\epsilon \delta))$.
\end{proof}

%------------------------------------------------------------------------------------------------------------------------------------------
\subsection{The Algorithm}

TODO

